Fast Trainable Projection for Robust Fine-Tuning

Robust fine-tuning aims to achieve competitive in-distribution (ID) performance while maintaining the out-of-distribution (OOD) robustness of a pre-trained model when transferring it to a downstream task. Recently, projected gradient descent has been successfully used in robust fine-tuning by constraining the deviation from the initialization of the fine-tuned model explicitly through projection. However, algorithmically, two limitations prevent this method from being adopted more widely, scalability and efficiency. In this paper, we propose a new projection-based fine-tuning algorithm, Fast Trainable Projection (FTP) for computationally efficient learning of per-layer projection constraints, resulting in an average $35\%$ speedup on our benchmarks compared to prior works. FTP can be combined with existing optimizers such as AdamW, and be used in a plug-and-play fashion. Finally, we show that FTP is a special instance of hyper-optimizers that tune the hyper-parameters of optimizers in a learnable manner through nested differentiation. Empirically, we show superior robustness on OOD datasets, including domain shifts and natural corruptions, across four different vision tasks with five different pre-trained models. Additionally, we demonstrate that FTP is broadly applicable and beneficial to other learning scenarios such as low-label and continual learning settings thanks to its easy adaptability. The code will be available at https://github.com/GT-RIPL/FTP.git.

==> algorithm_compare.tex <==
\begin{minipage}{0.46\textwidth}
\begin{algorithm}[H]
    \centering
    \caption{Schematic TPGM~\cite{tian2023trainable} at step $t$}\label{alg:tpgm}
    \begin{algorithmic}[1]
        \State $\mathbf{\Tilde{\mathbf{W}}}_t\gets\textbf{UGD}(\mathbf{W}_{t-1},\mathcal{D}_{tr}^t)$
        \State \colorbox{lime}{$\gamma_t\gets\textbf{ProjUpdate}(\gamma_t,\mathcal{D}_{val},\mathbf{\Tilde{\mathbf{W}}}_t,\mathbf{{\mathbf{W}}_0})$}
        \State $\mathbf{\mathbf{W}}_t\gets\textbf{Projection}(\gamma_t,\mathbf{\Tilde{\mathbf{W}}}_t,\mathbf{{\mathbf{W}}_0})$
    \end{algorithmic}
\end{algorithm}
\end{minipage}
\hfill
\begin{minipage}{0.46\textwidth}
\begin{algorithm}[H]
    \centering
    \caption{Schematic FTP at step $t$}\label{alg:ftp_short}
    \begin{algorithmic}[1]
        \State $\mathbf{\Tilde{\mathbf{W}}}_t,\mathbf{g}_t\gets\textbf{UGD}(\mathbf{W}_{t-1},\mathcal{D}_{tr}^t)$
        \State\colorbox{lime}{$\gamma_t\gets\textbf{ProjUpdate}(\gamma_t,\mathbf{g}_t,\mathbf{{\mathbf{W}}}_{t-1},\mathbf{{\mathbf{W}}_0})$}
        \State $\mathbf{\mathbf{W}}_t\gets\textbf{Projection}(\gamma_t,\mathbf{\Tilde{\mathbf{W}}}_t,\mathbf{{\mathbf{W}}_0})$
    \end{algorithmic}
\end{algorithm}
\end{minipage}



==> tables/clip_imagenet_wise.tex <==
\begin{table}[H]
\caption{ImageNet WISE Interpolation Result using CLIP ViT-Base Fine-tuned models. Following WISE~\cite{wortsman2022robust} We linearly interpolate the fine-tuned models from Tab.~\ref{tab:clip_imagenet} with the pre-trained CLIP model, sweeping interpolation rate $\in\{0.1,0.2,...,0.9\}$. The model with the best average accuracy$\uparrow$ is reported respectively for both fine-tuned models.
}
\centering

\resizebox{0.85\linewidth}{!}{
\begin{tabular}{c|c|cccc|cc} 

\toprule
&\multicolumn{1}{c|}{ID} & \multicolumn{4}{c|}{OOD} & \multicolumn{2}{c}{Statistics} \\


&ImageNet & ImageNetV2 & ImageNet-A &ImageNet-R & ImageNet-S&  OOD Average & Average\\

\midrule
WISE + FT & 80.94 &	72.47 &	33.18 &	\textbf{63.33} &	54.20  &	55.58	&60.82\\
WISE + FTP & \textbf{82.58}	& \textbf{74.10} &	\textbf{34.31}&	61.10&	\textbf{54.95}	&\textbf{56.12}&	\textbf{61.41}\\

\bottomrule		
\end{tabular}
}
\label{tab:clip_wise_imagenet}
\end{table}



